Building Time-Triggered Schedules for typed-DAG Tasks with alternative implementations

Hard real-time systems like image processing, autonomous driving, etc. require an increasing need of computational power that classical multi-core platforms can not provide, to fulfill with their timing constraints. Heterogeneous Instruction Set Architecture (ISA) platforms allow accelerating real-time workloads on application-specific cores (e.g. GPU, DSP, ASICs) etc. and are suitable for these applications. In addition, these platforms provide larger design choices as a given functionnality can be implemented onto several types of compute elements. HPC-DAG (Heterogeneous Parallel Directed Acyclic Graph) task model has been recently proposed to capture real-time workload execution on heterogeneous platforms. It expresses the ISA heterogeneity, and some specific characteristics of hardware accelerators, as the absence of preemption or costly preemption, alternative implementations and on-line conditional execution. In this paper, we propose a time-table scheduling approach to allocate and schedule a set of HPC-DAG tasks onto a set of heterogeneous cores, by the mean Integer Linear Programming (ILP). Our design allows to handle heterogeniety of resources, on-line execution costs, and a faster solving time, by exploring gradually the design space

==> texfiles/allocation.tex <==
\section{Allocation}
\label{sec:allocation}

% We consider the problem of allocating $n$ task specifications onto a
% given architecture $\mathsf{Arch} = \{e_1, \ldots, e_m\}$, consisting
% of $m$ engines, so that all timing constraints (minimum inter-arrival
% times and deadlines) are respected. Notice that only concrete tasks
% can be allocated to engines, however we often use the term
% \emph{allocating task specification} to express the whole process of
% allocating one of its concrete tasks.

\subsection{Allocation of task specifications}
\label{sec:vertex-allocation}

The goal of our methodology is to allocate a set of task
specifications into a set of engines, by selecting alternative
implementations, so that all tasks complete before their
deadlines. From an operational point of view, this is equivalent to
finding a feasible solution to a complex Integer Linear Programming
(ILP) problem. However, given the large number of combinations (due to
alternative nodes, condition-control nodes, and allocation decisions),
an ILP formulation of this problem fails to produce feasible solutions
in an acceptable time. Therefore, in this section we propose a set of
greedy heuristics to quickly explore the space of solutions.

Algorithm~\ref{algo:alloc-task-spec} describes the basic approach. The
algorithm can be customised with four parameters: $\mathsf{order}$ is
the sorting order of the concrete task sets (see Sections
\ref{sec:graph-spec-transf} and \ref{sec:graph-separation});
$\mathsf{slack}$ concerns the way the slack is distributed when
assigning intermediate deadlines and offsets (see Section
\ref{sec:artif-deadl-offs}); $\mathsf{alloc}$ can be best-fit (BF) or
worst-fit (WF); $\mathsf{omit}$ concerns the strategy to eliminate
sub-tasks when possible (see Section~\ref{sec:parallel-allocation}).

At each step, the algorithm tries to allocate one single task
specification (the $\mathsf{for}$ loop at line 5). For each task, it
first generates all concrete tasks (line 6), and sorts them according
to one relationship order ($\succ$ or $\gg$). For each concrete task,
it first assigns the intermediate deadlines and offsets according to
the methodology described in Section \ref{sec:artif-deadl-offs} (line
8), using one between the fair or the proportional slack
distributions. It separates the concrete tasks into tagged tasks
according to the corresponding tags (line 9).

The algorithm tries to allocate every tagged task onto single engines
having the corresponding tag (line 13) (this procedure is described
below in Algorithm \ref{algo:alloc-seq-spec}). If a feasible
allocation is found, the allocation is generated, and the algorithm
goes to the next specification task (line 14). If no feasible
sequential allocation can be found, the next concrete task is tested.

\begin{algorithm}[h]
  \caption{Allocation algorithm} \label{algo:alloc-task-spec}
  \begin{algorithmic}[1]
        \State \textbf{input :} $\taskset{}$: set of task specifications
        \State \textbf{parameters :} $\mathsf{order}$ ($\succ$ or $\gg$), $\mathsf{slack}$ (fair or proportional),
                     \\\hspace{2.07cm}$\mathsf{alloc}$ (BF or WF), $\mathsf{omit}$ (parallel or random)
        \State \textbf{output :} SUCCESS or FAIL
        \For {$\task{} \in \taskset{}$}
             \State $\Omega$ = generate\_and\_sort\_concrete\_task($\task{}, \mathsf{order}$)
             \For {$(\concrete{\task{}} \in \Omega)$}
                  \State assign\_deadlines\_offsets($\concrete{\task{}}$, $\mathsf{slack}$)
                  \State $\mathcal{S}(\concrete{\task{}})$ = filter\_tagged\_task($\concrete{\task{}}$)
             \EndFor
             \State allocated = \textbf{false}
             \For {$(\concrete{\task{}} \in \Omega)$}
                  % \State assign\_deadlines\_offsets($\concrete{\task{}}$, $\mathsf{slack}$)
                  % \State $\mathcal{S}(\concrete{\task{}})$=filter\_tagged\_task($\concrete{\task{}}$)
                  \If {(feasible\_sequential($\mathcal{S}(\concrete{\task{}})$, $\mathsf{alloc}$))}
                      \State  assign task to engines; allocated = \textbf{true};  \textbf{break};

                  \EndIf
              \EndFor
              \If {(\textbf{not} allocated)}
                 \For {($\concrete{\task{}} \in \Omega$)}
                     \State $(\concrete{\task{}}',\concrete{\task{}}'')$ = parallelize($\concrete{\task{}}$, $\mathsf{alloc}$, $\mathsf{omit}$)
                      \If {($\concrete{\task{}}' \neq \emptyset$)}
                          \State allocate $\concrete{\task{}}'$ to selected engines
                          \State add back $\concrete{\task{}}''$ to $\taskset{}$
                          \State allocated = \textbf{true}; \textbf{break} the loop
                      \EndIf
                \EndFor
                \State \textbf{if} (\textbf{not} allocated) \textbf{then} \textbf{return} FAIL
              \EndIf
         \EndFor
         \State \textbf{return} SUCCESS
  \end{algorithmic}
\end{algorithm}

The algorithm gives priority to single-engine allocations because they
reduce preemption cost, as discussed in
Section~\ref{sec:preempt-aware-sched}. In particular, by allocating an
entire tagged task onto a single engine, we reduce the number of null
sub-task to the minimum necessary, and so we can assign the cost of
preemption to fewer sub-tasks.

If none of the concrete tasks of a specification task can be allocated
(line 17), this means that one of the tagged tasks could not be
allocated on a single engine. Therefore, the algorithms tries to break
some of the tagged tasks of a concrete task into parallel tasks to be
executed on different engines of the same type. This is done by
procedure \textsf{parallelize}, which will be described in Section
\ref{sec:parallel-allocation}. In particular, one part of the concrete
task will be allocated, while the second part will be put back in the
list of not-yet-allocated task graphs (line 24). If this process is
also unable to find a feasible concrete task, the analysis fails (line
29).

\newcommand{\Input}[1]{\State {\bf input:}  #1}
\newcommand{\Output}[1]{\State {\bf output:} #1}
\vspace{-0.5em}
\subsection{Sequential allocation}
\label{sec:sequ-alloc}


Algorithm \ref{algo:alloc-seq-spec} tries to allocate a concrete task
on a minimal number of engines. It takes as input a set of tagged
tasks. For each tagged task, it selects the corresponding engines, and
sorts them according to parameter $\mathsf{alloc}$ (Best-Fit or
Worst-Fit utilization order). Then, it tests the feasibility of
allocating the tagged task on each engine in turn. If the allocation
is successful, the next tagged task is tested, otherwise the algorithm
tries the next engine. If the tagged task cannot be allocated on any
engine, the algorithm fails. If all tagged tasks have been allocated,
the corresponding allocation is returned.


% The feasibility of the couple task separation and the
% task separation set already allocated on the selected engine is tested
% in Line 8 (Theorem \ref{theo:single-engine-analys}). If the system is
% feasible, the allocation is stored and the loop is broken to proceed
% onto the allocation of the next task separation. If all engines of the
% same tag as the task separation to allocate has been investigated and
% the no-allocation is found, the allocation of the current concrete
% task is aborted on a fail. If all task separations can be feasibly
% allocated (Line 19), the stored allocations are returned and the
% process exits on SUCCESS. Feasibility test on Line 8 can be improved
% using utilization based necessary tests to further reduce the
% complexity.


\begin{algorithm}[h]
\caption{feasible\_sequential}\label{algo:alloc-seq-spec}
\begin{algorithmic}[1]
  \Input{$\mathcal{S}(\concrete{\task{}})$: set of tagged tasks, $\mathsf{alloc}$}
  \Output{feasibility: \textbf{SUCCESS} or \textbf{FAIL}}
  \For {$(\concrete{\task{}}({\mathsf{tag}}) \in \mathcal{S}(\concrete{\task{}}))$}
        \State engine\_list=select\_engine($\mathsf{tag}$)
        \State sort\_engines(engine\_list, $\mathsf{alloc}$) %\Comment Decr. U if $\mathsf{alloc}$=BF, else incr. U
        \State $f$ = \textbf{false}
        \State nfeas = 0
        \For {$(e \in  \mathsf{engine\_list})$}
               \State $f$ = dbf\_test($\concrete{\task{}} \cup \taskset_e$)
               \If {($f$)}
                   \State save\_allocation($\concrete{\task{}}$, $e$)
                   \State nfeas ++
                   \State {\bf break}
               \EndIf
        \EndFor
        \State \textsf{if} (\textbf{not} $f$) \textbf{then} \textbf{return} FAIL;
   \EndFor
   \If {(nfeas $= |\mathcal{S}(\concrete{\task{}})|$)}
         \State \textbf{return} SUCCESS, saved\_allocations
   \EndIf
  \end{algorithmic}
\end{algorithm}


\subsection{Parallel allocation}
\label{sec:parallel-allocation}

When the sequential allocation fails for a given task specification,
the algorithm tries to allocate one or more of its tagged tasks onto
multiple engines having the same tag. Algorithm
\ref{algo:paralleliz-concrete} takes as input a concrete task and two
parameters, $\mathsf{alloc}$ for BF or WF heuristics, and
$\mathsf{omit}$ to select which sub-task to remove first.

For each tagged task of the concrete task (line 5), the algorithm
selects the list of engines corresponding to the selected tag, and
sorts them according to BF or WF (line 7). Then, it tries to test the
feasibility of the tagged task on each engine (line 9). If the test
fails, it removes one sub-task from the tagged task and adds it to the
list of non allocated sub-tasks $\concrete{\tau}''$ (line 11). We
propose two heuristics:
\begin{enumerate}
\item \textbf{Random} heuristic: it selects a random sub-task and adds
  it to the omitted list.
\item \textbf{Parallel} heuristic: to be feasible, the critical path
  of each tagged task must be feasible on a unlimited number of
  engines. Thus, we are starts by removing sub-tasks that do not
  belong to the critical path as they may be the ones causing the
  non-feasibility (here we assume that sequential allocation has
  failed). Thus, vertices not belonging to the critical path are
  omitted first. Once a vertex is omitted, one if its predecessors or
  successors are omitted further in priority to maximize the size of
  maximal sequential subsets.
\end{enumerate}
The feasibility test is repeated until a feasible subset of
$\concrete{\tau}(\mathsf{tag})$ is found. The omitted tasks are tried
on the next engine with the same tag (line 16). At the end of the
procedure, two concrete tasks are produced: $\concrete{\tau}'$ is the
feasible part that will be allocated, while $\concrete{\tau}''$ will
be tried again in the following iteration of Algorithm
\ref{algo:alloc-task-spec}.

% further it selects engines and sort them in the same logic as
% sequential allocation. Further, it tests the allocation of the tagged
% tasks one by one. If the system is not feasible the algorithm omits a
% certain number of sub-tasks and retries the allocation until finding a
% feasible schedule. At worst cases, the algorithm will remove all
% sub-tasks hence the task demand bound function is zero, thus the
% system is trivially feasible. In this case, the algorithm interate on
% the previous step on other engines if available. If all engines has
% been investigated without finiding a feasible schedule, the algorithm
% exists on FAIL and further the main algorithm (Algorithm
% \ref{algo:alloc-task-spec}) will try another concrete task. If the
% algorithm exits on succes, the allocation is saved, and omitted
% sub-tasks are used to build an isomorphic task to the original tagged
% task. The isomorphic just-built task is put back onto the non
% allocated task list to be allocated in future iterations.

% The omit sub-tasks operation is the key function. One may try all
% possible sub-tasks looking for an optimal solution. We propose to use
% $2$ heuristics:

\begin{algorithm}[h]
\caption{parallelize}\label{algo:paralleliz-concrete}
\begin{algorithmic}[1]
  \Input{$\concrete{\task{}}$: concrete task, $\mathsf{alloc}$ (BF or WF),}
         \\\hspace{0.95cm} $\mathsf{omit}$ (parallel or random)
  \Output{concrete tasks $(\concrete{\tau}', \concrete{\tau}'')$}%or \textbf{FAIL}}

  \State{$\concrete{\tau}' = \emptyset, \concrete{\tau}''=\emptyset$}
  \For {$(\concrete{\task{}}(\mathsf{tag}) \in  \mathcal{S}(\concrete{\task{}}))$}
      \State engine\_list=select\_engines(tag)
      \State sort(engine\_list, $\mathsf{alloc}$)
      \For {$(e \in  \mathsf{engine\_list})$}
          \State $f$=dbf\_test($\concrete{\task{}}(\mathsf{tag}) \cup \taskset_{e}$)
          \While {(\textbf{not} $f$) }
             \State $\concrete{\tau}''$ = $\concrete{\tau}'' \cup$ remove($\concrete{\task{}}(\mathsf{tag}),\mathsf{omit}$)
             %\State save\_omitted\_sub-tasks
             \State $f$=dbf\_test($\concrete{\task{}}(\mathsf{tag}) \cup \taskset_{\mathsf{E}}$)
          \EndWhile
          \If {($\concrete{\task{}}(\mathsf{tag}) \neq \emptyset$ )}
             \State $\concrete{\tau}' = \concrete{\tau}' \cup$ save\_allocation($\concrete{\task{}}(\mathsf{tag}),e$)
             \State $\concrete{\tau}(\mathsf{tag}) = \concrete{\tau}'', \concrete{\tau}'' = \emptyset$
             \State allocated = \textbf{true}
             \State \textbf{break}
          \EndIf
      \EndFor
      \State \textbf{if} (\textbf{not} allocated) \textbf{return} $\emptyset, \concrete{\tau}$
 \EndFor
% \State rej\_task = construct\_task\_from save\_allocations
 \State \textbf{return} $\concrete{\tau}', \concrete{\tau}''$
\end{algorithmic}
\end{algorithm}

% \subsection{Workflow}\label{sec:workflow}

% On the point of view of the implementation, the main idea is to
% construct a workflow as described in Figure
% \ref{fig:work-flow}. The platform description (see Section \ref{sec:architecture-model})
% and the taskset (see Section \ref{sec:task-model}) we wish to allocate and analyze are passed as inputs
% for our heuristic-based allocation strategy.
% After that the necessary scheduling parameters are assigned for each node of the input graphs,
% the previously described allocation algorithms will be performed for providing the sufficient
% schedulability tests. If at least a feasible solution is found,
% task-engine allocation data structure and the source code for kernels
% and applications are used to produce binary executables. In an online
% phase, these executables are able to meet the timing constraints
% imposed in the offline phases.

% \begin{figure}[h]
%   \centering
%   \resizebox{\columnwidth}{!}{
%     \input{figs/work_flow.tex}
%     }
%   \caption{Workflow diagram}
%   \label{fig:work-flow}
% \end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nv_paper"
%%% End:


==> texfiles/conclu.tex <==
\section{Conclusions and future work}
\label{sec:concl-future-work}

In this paper, we presented the HPC-DAG real-time task model, which
allows specifying both off-line and on-line alternatives of a task
instance, to fully exploit the heterogeneity of complex embedded
platforms. We also presented a schedulability analysis and a set of
heuristics to allocate HPC-DAGs on heterogeneous computing
platforms. The analysis takes into account the cost of preemption,
which may be non-negligible in certain specialized engines. As a
future work, we are considering extending our framework to account for
the memory interference between different compute
engines.% , as it is known to cause significant variations in
% execution times~\cite{ali2017protecting, cavicchioli2017memory}


% For studying the real time behavior of task sets described with our proposed model,
% we presented a set of heuristics and related feasibility tests.
% These heuristics refers to how we assign deadlines and how we allocate sub-tasks to
% engines having different ISAs and our test methodologies was able to study
% how different heuristics perform on generated tasksets.
% The goal is to provide a formally sound workflow that takes as input a platform
% description and the task set and outputs a set of workloads to dispatch to
% the engines. Our target platform features different kind of accelerators, hence
% different preemption policies and costs are in place: for these reasons, a novel
% preemption cost aware approach has been exploited for feasibility tests.
% Results of our extensive synthetic simulations show that a significant
% reduction in pessimism occurs with our proposed approach. This leads to
% an increase in resource utilization compared to similar approaches in
% the literature.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nv_paper"
%%% End:


==> texfiles/results.tex <==
\section{Results and discussions}
\label{sec:results}
\definecolor{cl1}{HTML}{E41A1C}
\definecolor{cl2}{HTML}{377EB8}
\definecolor{cl3}{HTML}{4DAF4A}
\definecolor{cl4}{HTML}{984EA3}


\begin{figure*}[t]
  \begin{subfigure}[b]{0.35\textwidth}
    \resizebox{0.8\columnwidth}{!}{
      \begin{tikzpicture}
        \begin{axis}
          [axis x line=bottom, axis y line = left, xlabel={Total
            Utilization index}, ylabel={Schedulability rate},
          % xmin = 200.0,
          % xmax = 4.5, ymin = 0, ymax = 35,
          y label style={at={(axis description cs:-0.07,.5)},rotate=0,anchor=south},
          legend entries={BRF-P,BOF-P, BRF-R,BOF-R,WRF-P,WOF-P,  BOP-P,BRP-P,WOP-P,WRP-P,CP-DAG}, legend
          style={at={(-0.15,1)}}, ]
          \addplot [mark=diamond*,black]table[y index=4,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=square*,blue]table[y index=2,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=diamond*,blue,dashed]table[y index=10,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=square*,red,dashed] table[y index=9,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=diamond,black] table[y index=8,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=square,blue] table[y index=6,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=triangle*,red] table[y index=1,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=*,cl3]table[,y index=3,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=triangle,red] table[y index=5,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=o,cl3] table[y index=7,x index=0]{res/sched_rate_0.6_par.dat};
          \addplot [mark=o,yellow] table[y index=1,x index=0]{res/ml_r.dat};
        \end{axis}
      \end{tikzpicture}
    }
    \caption{Schedulability rate VS util.}\label{fig:sched-rate}
  \end{subfigure}
  \begin{subfigure}[b]{0.35\textwidth}
    \resizebox{0.8\columnwidth}{!}{
      \begin{tikzpicture}
        \begin{axis}
          [ axis x line=bottom, axis y line = left, xlabel={Total
            Utilization index}, ylabel={\# active CPUs},
          y label style={at={(axis description cs:-0.07,.5)},rotate=0,anchor=south},
          legend entries={BRF-P,BOF-P, WRF-P,WOF-P,  BOP-P,BRP-P,WOP-P,WRP-P}, legend
          style={at={(1.45,1)}}, ]
          \addplot [mark=diamond*,black]table[y index=4,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=square*,blue]table[y index=2,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=diamond,black] table[y index=8,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=square,blue] table[y index=6,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=triangle*,red] table[y index=1,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=*,cl3]table[,y index=3,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=triangle,red] table[y index=5,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=o,cl3] table[y index=7,x index=0]{res/avg_ncore_0.6_par.dat};
          \addplot [mark=o,yellow] table[y index=1,x index=0]{res/ml_a_c.dat};
        \end{axis}
      \end{tikzpicture}
    }
    \caption{\#Active CPUS vs util.}\label{fig:active_cores}
  \end{subfigure}
  \begin{subfigure}[b]{0.35\textwidth}
    \resizebox{0.8\columnwidth}{!}{
      \begin{tikzpicture}
        \begin{axis}
          [ axis x line=bottom, axis y line = left, xlabel={Total
            Utilization index}, ylabel={active CPUs utilization},
          % xmin = 200.0,
          % xmax = 4.5, ymin = 0, ymax = 35,
          y label style={at={(axis description cs:-0.07,.5)},rotate=0,anchor=south},
          legend entries={BRF-P,BOF-P, WRF-P,WOF-P,  BOP-P,BRP-P,WOP-P,WRP-P}, legend
          style={at={(1.45,1)}}, ]
          \addplot [mark=diamond*,black]table[y index=4,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=square*,blue]table[y index=2,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=diamond,black] table[y index=8,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=square,blue] table[y index=6,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=triangle*,red] table[y index=1,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=*,cl3]table[,y index=3,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=triangle,red] table[y index=5,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=o,cl3] table[y index=7,x index=0]{res/avg_u_a_0.6_par.dat};
          \addplot [mark=o,yellow] table[y index=1,x index=0]{res/ml_a_u.dat};
        \end{axis}
      \end{tikzpicture}
    }
    \caption{Active CPU util. VS tot. util. }\label{fig:acti-u-c}
  \end{subfigure}

\end{figure*}





In this section, we evaluate the performance of our scheduling
analysis and allocation strategies. We compare against the 
CP-DAG model proposed by Melani et al. in \cite{melani_bertogna}, which 
adopted a global scheduling approach, whereas our analysis is based on
partitioned scheduling. Therefore, we extended the CP-DAG model to
support multiple engines. Moreover, we applied the same allocation
heuristics of Section \ref{sec:allocation} and the same scheduling
analysis of Section \ref{sec:analysis} to HPC-DAGs and to CP-DAG.

% we adapted the analysis
% of~\cite{melani_bertogna} to support partitioned scheduling and
% heterogeneous architectures.
% %% TODO: How ?

In the following experiments, we considered the NVIDIA Jetson AGX
Xavier platform\footnote{
  \url{https://elinux.org/Jetson_AGX_Xavier}}. It features 8 CPU cores
and four different kinds of accelerators: one discrete and one
integrated GPU, one DLA and one PVA. Each accelerator is treated as a
single computing resource. In this way, we can exploit task level
parallelism as opposed to allowing the parallel execution of more than
one sub-task to partitions of the accelerators (e.g., at a given time
instant, only one sub-task is allowed to execute in all the computing
clusters of a GPU).

\subsection{Task Generation}
\label{sec:task-generation}

We apply our heuristics on a large number of randomly generated
synthetic task sets.

The task set generation process takes as input an engine/tag
utilization for each tag on the platform. First, we start by
generating the utilization of the $n$ tasks by using the
UUniFast-Discard \cite{uni} algorithm for each input
utilization. Graph sub-tasks can be executed in parallel, thus task
utilization can be greater than 1. The sum of every per-tag
utilization is a fixed number upper bounded by the number of engines
per tag.

The number of nodes of every task is chosen randomly between 10 and
30. We define a probability $p$ that expresses the chance to have an
edge between two nodes, and we generate the edges according to this
probability. We ensure that the graph depth is bounded by an integer
$d$ proportional to the number of sub-tasks in the task. We also
ensure that the graph is \emph{weakly connected} (i.e. the
corresponding undirected graph is connected); if necessary, we add
edges between non-connected portions of the graph. Given a sub-task
node, one of its successors is an alternative node or a conditional
node with a probability of $0.7$.

To avoid untractable hyper-periods, the period of every task is
generated randomly according to values taken from a list, where the
minimum is $120$ and the maximum is $120,000$. For every sub-task, we
randomly select a tag. Further, for each tag, we use algorithm
UUniFAST-Discard again to generate single sub-task utilization. Thus,
the sub-task utilization can never exceed 1. Further, we multiply the
utilization of each sub-task by the task period to generate the vertex
execution time. A CP-DAG is generated from a HPC-DAG by selecting one
of the possible concrete tasks at random.

\subsection{Simulation results and discussions}

We varied the baseline utilization from $0$ to the number of engines
per engine tag in $16$ steps. Therefore, the step size vary from one
engine tag to the other: the step size is $0.5$ for CPUs, and $0.0625$
for the others. For each utilization, we generated a random number of
tasks between 20 and 25.

The results are presented as follows. Each algorithm is described
using $3$ letters: (i) the first is either $\mathsf{B}$ for best fit
or $\mathsf{W}$ for worst first allocation techniques; (ii) the second
is either $O$ for the $\succ$ order relation, or $R$ for the $\gg$
order relation; (iii) the third describes the deadline assignment
heuristic, $F$ for fair and $P$ for proportional. The algorithm name
may also contain either option $P$ for the parallel allocation
heuristic that eliminates parallel nodes first, or $R$ for the random
heuristic which randomly selects the sub-task to remove.  Average
values for $85$ simulations per utilization step are presented.

Figure \ref{fig:sched-rate} represents the schedulability rate of each
combination of heuristics cited above as a function of the total
utilization. The fair deadline assignment technique presents better
schedulability rates compared to proportional deadline assignment. In
general, BF heuristic combinations outperform WF heuristic: this can
be explained by observing that BF tries to pack the maximum number of
sub-tasks into the minimum number of engines, allowing more
flexibility to schedule \emph{heavy} tasks on other engines.

In the figures, the CP-DAG model proposed in \cite{melani_bertogna} is
shown in yellow. Since the CP-DAG has no alternative implementations,
the algorithm has less flexibility in allocating the
sub-tasks. Therefore \emph{by construction} the results for HPC-DAG
dominate the corresponding results for CP-DAG. However, it is
interesting to measure the difference between the two models: for
example, in Figure \ref{fig:sched-rate} the difference in the
schedulability rate between the two models is between 10\% and 20\%
for utilization rates between 6 and 14.

When the system load is low, all combinations of heuristics allow
high schedulability rates. BRF outperforms the others because
it aims at relaxing the utilization of scarce engines, thus
avoiding the unfeasibility of certain task sets due to a high load on
scarce engines. % (DLA and PVA/ GPUs)
However, when dealing with high loads, BOF presents better
schedulability rates, as it reduces the execution overheads on all
engines.

Figure \ref{fig:active_cores} reports the average number of active
cores (CPUs) as a function of the total utilization. WF-based
heuristics use always all cores, as we generate at least $15$ CPU
subtasks, i.e., the number of tasks is larger than the number of CPUs. BF
heuristics allows packing the maximum number of sub-tasks on the
minimum number of engines, thus the utilization increases
quasi-linearly. This occurs until the maximum schedulability limit is
reached% (i.e. number of cores)
. BRF heuristic uses more CPU cores
because it \emph{preserves} the scarce resources, thus it uses more
CPU engines. As BOF privileges reducing the overall load, it reduces
the load on the CPUs compared to BRF.

Figure \ref{fig:acti-u-c} shows the average active utilization for
CPUs. As expected, average utilization of BF-based heuristics is
higher compared to WF. Again, BRF has higher utilization than BOF
because it schedules more workload on CPU cores than the other
heuristics. As the workload is equally distributed on different CPUs,
the WF heuristics may be used to reduce the CPUs operating frequency
to save dynamic energy. Regarding BF heuristics, we see that BRF is
not on the top of the average load because it uses more cores than the
others.

% \begin{figure}[t]
%   \centering
%   \resizebox{0.65\columnwidth}{!}{
%     \begin{tikzpicture}
%       \begin{axis}
%         [
%         axis x line = bottom,
%         axis y line = left,
%         xlabel={Total Utilization index},
%         ylabel={Average scarce-engine utilization},
%         y label style={at={(axis description cs:-0.07,.5)},rotate=0,anchor=south},
%         legend entries={BRF-P,BOF-P, WRF-P,WOF-P,  BOP-P,BRP-P,WOP-P,WRP-P},
%         legend style={at={(1.45,0.7)}},
%         ]
%         \addplot [mark=diamond*,black]table[y index=1,x index=0]{res/avg_u_sc_0.6_par.dat};
%         \addplot [mark=square*,blue]table[y index=2,x index=0]{res/avg_u_sc_0.6_par.dat};
%         \addplot [mark=diamond,black] table[y index=3,x index=0]{res/avg_u_sc_0.6_par.dat};
%         \addplot [mark=square,blue] table[y index=4,x index=0]{res/avg_u_sc_0.6_par.dat};
%         \addplot [mark=o,yellow] table[y index=1,x index=0]{res/ml_a_u_s.dat};
%       \end{axis}
%     \end{tikzpicture}
%   }
%   \caption{DLA, GPUs, PVA utilizations  vs  total utilization.}\label{fig:sc_a_u}
% \end{figure}

% Figure \ref{fig:sc_a_u} shows the average utilization of the scarce
% resources. As you may notice, order relation $\gg$ based heuristics
% allows to reduce the load on the scarce resources compared to
% $\succ$. In fact, the higher is the load, the less loaded are the
% scarce resources.


\subsection{Preemption cost simulation}
\label{sec:preempt-cost-simul}


\begin{figure}[h]
  \centering
  \resizebox{0.65\columnwidth}{!}{
    \begin{tikzpicture}
      \begin{axis}
        [
        axis x line = bottom,
        axis y line = left,
        xlabel={Total Utilization index},
        ylabel={Schedulability rates},
        y label style={at={(axis description cs:-0.07,.5)},rotate=0,anchor=south},
        legend entries={MAX-PREEMP,REDUCED-PREM},
        legend style={at={(1.25,1)}} ]
        \addplot [mark=diamond*,black]table[y index=1,x index=0]{res/preemp.dat};
        \addplot [mark=square*,blue]table[y index=2,x index=0]{res/preemp.dat};
      \end{axis}
    \end{tikzpicture}
  }
  \caption{Preemption cost Theorem vs max}\label{fig:preemp_cost}
\end{figure}

In all previous experiments, we applied the analysis described in
Section~\ref{sec:preempt-aware-sched} to account for preemption
costs. In particular, we applied the technique of
Theorem~\ref{theo:preempt-all}, by assuming that the cost of
preempting a sub-task is 30\% of the sub-task execution time on a GPU,
10\% on DLA and PVA, and 0.02\% on the CPUs. These are representative numbers
experimented in real settings. DLA and PVA are
non-preemptable engines. However, longer jobs might be split into
smaller chunks, translating to a splitting overhead due to the
submission of multiple kernel calls instead of a single batch of
commands.


To highlight the importance of a proper analysis for preemption costs,
We report in Figure \ref{fig:preemp_cost} the schedulability rates
obtained by BRF-P in two cases: when considering the analysis of
Lemma~\ref{theo:worst_preemption}, where the maximum preemption cost
is charged to all preempting sub-tasks, and that of Theorem
\ref{theo:preempt-all}, where the cost is only charged to one of the
sub-tasks in the maximal sequential subset. As the utilization increases,
the schedulability drastically falls for the first method, while the analysis
of Theorem \ref{theo:preempt-all} allows tighter schedulability rates.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nv_paper.tex"
%%% End:



==> texfiles/stat.tex <==
\section{Related work}
\label{sec:related-work}

Many authors
\cite{qamhieh2013global,melani_bertogna,saifullah_multi-core_2013,li2014analysis,saifullah2012real,fonseca2016response,Marinca:2004:ADA:2285761.2285882,peppehoussemJSA,houssamPeppeRTNS}
have proposed real-time task models based on DAGs. % Usually, vertices
% model sub-tasks and edges model the precedence order between them in
% the same logic as our model (see Section \ref{sec:task-model}).
However, to the best of our knowledge, none of
the existing models supports alternative implementations of the same
functionality on different computing engines.

In \cite{Marinca:2004:ADA:2285761.2285882}, the
deadline assignment problem is addressed for distributed real-time systems. 
Two algorithms are proposed, i.e., Fair Laxity Distribution (FLD) and Unfair Laxity Distribution (ULD),
evaluating their impact on the schedulability of the system. In
\cite{li2014analysis}, a schedulability analysis is proposed for a set of DAGs 
scheduled with global EDF, global rate-monotonic (RM), and federated scheduling. 
In \cite{wu2014deadline}, a general framework is presented for
partitioning real-time tasks onto multiple cores using resource
reservation. A technique is proposed to set
task activation times and deadlines, using an ILP
formulation to solve the allocation and assignment problems. However,
these approaches may be very time consuming when applied to applications consisting of
tens or hundreds of sub-tasks.

A response time analysis for partitioned fixed-priority DAG tasks is presented in
\cite{fonseca2016response}. DAGs are modeled as a set of self-suspending tasks, 
characterizing their worst-case scheduling scenario.

In \cite{melani_bertogna}, conditional nodes have been introduced to 
DAG tasks for modeling conditional branches. Different methods
are presented to compute upper-bounds on the response-time under global scheduling.
In \cite{stigge2011digraph}, alternative
on-line execution patterns can be expressed using
\emph{digraph}s. However, the digraph model cannot express parallelism
and it only supports sequential tasks. In
\cite{mutlimode}, an extension is presented to model parallel workloads within digraphs.
However, none of these models is able to express alternative implementations of a task on heterogeneous engines.

Regarding scheduling algorithms to be adopted within the heterogeneous engines
of modern embedded platforms, a key factor to  consider is the cost of preemptions,
which may be non negligible, especially for GPU engines. 
Initial work on preemptive GPU scheduling 
assumed that preemption was viable at the kernel granularity
\cite{zhong2013kernelet}. Preemption for GPU Kernels in NVIDIA
architectures are nowadays natively supported, both via hardware and
software mechanisms, starting from the Maxwell architecture (released
in 2014). In \cite{amert2017gpu} and \cite{capodieci2017sigamma},
the concept of CUDA stream preemption is detailed. A stream in a CUDA
application is a queue of implicitly synchronized kernel and copy
operations, so that if a kernel on a stream is currently running
within the GPU's computing clusters, offloading a kernel on a higher
priority stream will cause preemption at CUDA thread block
boundaries. The Pascal architecture (released in 2016) increased the
preemption granularity to kernel instruction boundaries among kernels
belonging to different applications \cite{capodieci2018work}. This finer 
preemption granularity was exploited in \cite{capodieci2018deadline} 
to present a closed source EDF scheduler prototype. Preemption of GPU kernels can also be
achieved without modifying the proprietary GPU drivers: preemption
points might be manually inserted into kernels in the form of a
system-accessible memory location to query during kernel execution. In
this case, context save and restore operations must also be
implemented by the application developer, either manually or through
automatic code instrumentation. Several contributions exist that
exploit such mechanisms
\cite{hartmann2019gpuart,calhoun2012preemption,chen2017effisha}.
Another approach for obtaining preemption is by exploiting persistent
threads \cite{wu2017flep}.  Such methodologies can be used for
architectures and APIs other then NVIDIA's (e.g. Khronos' OpenCL
\cite{chiu2018enabling}). More recently, other device vendors started
to natively support preemption at an architectural level, e.g., AMD
devices \cite{acharya2019primitive} and Intel iGPUs
\cite{junkins2015compute}. Depending on the computing architecture and
on the nature of the workload, GPU tasks present different degrees of
preemption granularity and related preemption costs. The cost of
preempting an executing context on a GPU might present significant
differences, as it will involve saving and restoring contexts of
variable size and/or reaching the next viable preemption point.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nv_paper.tex"
%%% End:

